Astrometric Microlensing by Primordial Black Holes with The Roman Space Telescope

Primordial Black Holes (PBHs) could explain some fraction of dark matter and shed light on many areas of early-universe physics. Despite over half a century of research interest, a PBH population has so far eluded detection. The most competitive constraints on the fraction of dark matter comprised of PBHs ($f_{\rm DM}$) in the $(10^{-9}-10)M_{\odot}$ mass-ranges come from photometric microlensing and bound $f_{\rm DM}\lesssim10^{-2}-10^{-1}$. With the advent of the Roman Space Telescope with its sub-milliarcsecond (mas) astrometric capabilities and its planned Galactic Bulge Time Domain Survey (GBTDS), detecting astrometric microlensing signatures will become routine. Compared with photometric microlensing, astrometric microlensing signals are sensitive to different lens masses-distance configurations and contains different information, making it a complimentary lensing probe. At sub-mas astrometric precision, astrometric microlensing signals are typically detectable at larger lens-source separations than photometric signals, suggesting a microlensing detection channel of pure astrometric events. We use a Galactic simulation to predict the number of detectable microlensing events during the GBTDS via this pure astrometric microlensing channel. Assuming an absolute astrometric precision floor for bright stars of 0.1 mas for the GBTDS, we find that the number of detectable events peaks at $\approx 10^{3} f_{\rm DM}$ for a population of $ 1 M_{\odot}$ PBHs and tapers to $\approx 10f_{\rm DM}$ and $\approx 100f_{\rm DM}$ at $10^{-4}M_{\odot}$ and $10^{3}M_{\odot}$, respectively. Accounting for the distinguishability of PBHs from Stellar lenses, we conclude the GBTDS will be sensitive to a PBH population at $f_{\rm DM}$ down to $\approx10^{-1}-10^{-3}$ for $(10^{-1}-10^{2})M_{\odot}$ likely yielding novel PBH constraints.

==> scratch.tex <==
%each of these constraints entails its own assumptions and systematics, typically relying on a monochromatic mass function for the PBH population \citep[although not necessarily, e.g.,][]{Franciolini2021}.
%The observational signatures range from observations of the cosmic microwave background measurements~\citep[e.g.,][]{Ricotti2007} to gravitational wave observations of merging BHs~\citep[e.g.,][]{Franciolini2021} to gravitational microlensing.

(originally termed Massive Compact Halo Object or MACHOs, which contain PBH populations as a subset) started with the MACHO~\citep{Alcock2001}, EROS~\citep{Tisserand2006,Blaineau2022} and OGLE~\citep{Wyrzykowski2009,Wyrzykowski2010,Wyrzykowski2011a,Wyrzykowski2011b} collaborations. 
These different collaborations observed the large and small Magellanic clouds (LMC and SMC, respectively) starting in the 1990's and continuing through the 2000's. 

These different collaborations observed the large and small Magellanic clouds (LMC and SMC, respectively) starting in the 1990's and continuing through the 2000's. 

This initial work was followed by the Subaru Hyper Suprime-Cam (HSC) survey observing M31, which instead focused on a range of masses in the substellar regime ($10^{-14}-10^{-9} M_{\odot}$) due to the much faster survey cadence (therefore sensitive to shorter timescale microlensing events). 
Constraints from this survey ranged on the order of $f_{\rm DM} \sim 0.1-1\%$~\citep{Niikura2019a}.
In addition to the HSC survey, recent work has also utilized past OGLE data of the galactic bulge~\citep{Mroz2017}, placing constraints on the dark matter fraction at $f_{\rm DM}\sim 1-10\%$~\citep{Niikura2019b} for a mass range of $10^{-6}-10^{-3} M_{\odot}$.


For reference, we can compare against the estimate of detectable \emph{photometric} and astrometric PBH events are accessible to GBTDS, courtesy of \citet{Pruett2022} (at $30M_{\odot}$).
At this mass, we can expect to be $2-3\times$ more sensitive than a photometric-only search.
\perkins{More takeaway points? Need to hammer home the importance of astrometric over photometric more?}


%Fig.~\ref{fig:observables} shows where the detectable PBH events lie in the astrometric microlensing observable space ($\theta_{E},\pi_{E},t_{E}$) relative to the astrophysical lens population. Generally, as the PBH mass increases, $\theta_{E}$ and $t_{E}$ increase and  $\pi_{E}$ decreases because they are $\propto\sqrt{M}$ and $\propto 1/\sqrt{M}$, respectively (see Eq.~\eqref{eq:theta_E} and Eqs.~\eqref{eq:tE_piE}). PBHs lie along straight lines of constant mass in the $\theta_{E}-\pi_{E}$ space of Fig. \ref{fig:observables} because we injected populations with monochromatic mass distributions. 

As mentioned above, the astrophysical populations used in \texttt{PopSyCLE} do not include objects below roughly $10^{-1} M_{\odot}$, leading to an over-sensitivity of this distance measure to PBH populations in this mass range, which was less severe for the Hellinger distance.

%\footnote{\perkins{Possibly too much detail, just writing it down for reference while writing the text.} Note that this is very related to the concept of the purity of samples, the difference being that the purity is the integral of the (unnormalized) posterior probability. I.e., the purity could be used to define a ``unique'' region by optimizing the region $\mathcal{M}$ such that ${\rm Purity} \equiv \int_\mathcal{M} p({\rm PBH}) p(  t_E, \theta_E | {\rm PBH}) d t_E d \theta_E / \int_{\mathcal{M}} p(t_E, \theta_E) d t_E d \theta_E = {\rm threshold} $, which has a different but similar interpretation to the current method in this work.}


%All quantities are shown for different PBH lens class probabilities \citep[$p(\text{class}_{{\text{PBH}}}|t_{E},\theta_{E})$; see section 3.2 of][]{Perkins2023} thresholds of $0.5$, $0.9$ and $0.95$. Fig. \ref{fig:}



%First, we compute the similarity between the intrinsic distribution of simulated events in $t_{E}-\theta_{E}$-space between the distribution of astrophysical and PBH lens ($P$) and just astrophysical lenses ($Q$), using the Hellinger distance, 
%While a direct comparison of the distribution of observables assuming the lenses belong to the PBH population, mathematically $p(t_E, \theta_E | {\rm PBH})$, and the distribution predicted by assuming the lenses are astrophysical, mathematically $p(t_E, \theta_E | {\rm Astro})$, can be illuminating, this would not directly incorporate our prior information that astrophysical lenses outnumber PBH lenses by a wide margin ($p({\rm Astro}) > p({\rm PBH}))$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Scott's modifications
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%While a direct comparison of the distribution of observables assuming the lenses belong to the PBH population, mathematically $p(t_E, \theta_E | {\rm PBH})$, and the distribution predicted by assuming the lenses are astrophysical, mathematically $p(t_E, \theta_E | {\rm Astro})$, can be illuminating, this is more related to identifying individual events as involving a PBH or astrophysical lens.
%Before discussing analyses addressing that question, we would first like to focus on the question of distinguishability between a lens population model that incorporates PBH lenses and one that does not.
%*************


%This question is one of model comparison (at the population level) and speaks to the effectiveness of \emph{statistical} tools to detect a subpopulation of PBHs (e.g., see results related to the measurements of abundances and Bayes' factors in \citet{Perkins2023}).
%Mathematically, the two models being considered will be one conditioned on an astrophysical-only population of lenses given by $p(t_E,\theta_E| {\rm Astro})$ and a model including both astrophysical and primordial populations given by the population-model evidence $p(t_E, \theta_E ) \equiv p({\rm PBH}) p(t_E,\theta_E | {\rm PBH}) +p({\rm Astro}) p(t_E,\theta_E | {\rm Astro})$, i.e., the probability of an event with parameters $t_E$ and $\theta_E$ marginalized over both possible classes.
%To quantify the distinguishability between these two models from an intrinsic point of view (i.e., neglecting observational uncertainties), the Hellinger distance can be calculated between the two predictions for the distribution of event observables, which is defined as
%First, we compute the similarity between the intrinsic distribution of simulated events in $t_{E}-\theta_{E}$-space between the distribution of astrophysical and PBH lens and just astrophysical lenses, using the Hellinger distance, 

%\begin{equation}
%    H^{2}(P,Q) = \frac{1}{2}\int{\left(\sqrt{P()}-\sqrt{Q}\right)}d\theta_{E}dt_{E}.
%    \label{eq:hellinger}
%\end{equation}
%
%\begin{equation}
%    H^{2} = \frac{1}{2}\int{\left(\sqrt{p_{\tiny {\rm PBH}\cup{\rm astro}}(t_E, \theta_E  )}-\sqrt{p_{ \tiny {\rm astro}}(t_E, \theta_E) }\right)^2}d\theta_{E}dt_{E}.
%    \label{eq:hellinger}
%\end{equation}

%\begin{equation}
%    H^{2} = 1-\int{\sqrt{p(t_E, \theta_E  )p(t_E, \theta_E | {\rm Astro} )  }}d\theta_{E}dt_{E}\,.
%    \label{eq:hellinger}
%\end{equation}
%where $p(t_E, \theta_E | {\rm Astro})$ is the likelihood of seeing an event with $t_E$ and $\theta_E$ given it involved an astrophysical lens. Meanwhile, $p(t_E, \theta_E)$ is the class evidence of $t_E$ and $\theta_E$, or the probability of an event marginalized over both classes. This is mathematically given by $p(t_E, \theta_E) \equiv p({\rm PBH}) p(t_E,\theta_E | {\rm PBH}) +p({\rm Astro}) p(t_E,\theta_E | {\rm Astro})$. A comparison of these two distributions (the class evidence and the likelihood conditioned on the lens being astrophysical) helps to quantify the distinguishability of the model built on the assumption that all lenses are astrophsyical and the different models that include a subpopulation of PBH lenses at different masses. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%\begin{figure}
%    \centering
%    \includegraphics{figs/tE_piE_thetaE_scatters.png}
%    \caption{Caption}
%    \label{fig:enter-label}
%\end{figure}
%I think we are going to have to drop this due to time constraints
%\subsection{Lenses with multiple %events}\label{sec:multipleLenses}

%Finally, we consider objects that lens multiple sources, allowing for precision measurements of their properties.
%This type of observation is only possible with a multi-year survey and high precision astrometry, without considering targeted follow-up observations.
%The RGBTDS brings this possibility to reality, and we therefore consider this in the context of PBH events.

%In Fig.~\ref{fig:lens_multiple_sources}, we can see that the number of PBH events with multiple, independent sources (i.e., not close-binary sources) increases with increasing PBH mass. 
%Similar to arguments made in Sec.~\ref{sec:event_rates}, this is attributable to the fact that larger lenses have larger Einstein-radii, yielding higher probabilities of lensing.
%Furthermore, we also see in Fig.~\ref{fig:lens_multiple_sources} %that the distribution of lenses with multiple, independent %sources is reaches to greater distances, just as in the case of %single-source events.

%\perkins{it would be interesting to show how much improved the %constraints on lensing parameters is for multiple-source lenses %compared to single source lenses. Just some fisher calculation. }

%\begin{figure}
    %\centering
    %\includegraphics{figs/Distance_Dupe_Histogram_markerlast.pdf}
    %\caption{
    %Stacked histogram of the distance to the lens for lenses that lens multiple sources during GBTDS. Over plotted is the distribution of Astrophysical lenses that also cause multiple events. The majority of the multiple source events%are caused by nearby lenses with $\approx2$kpc.
%    }\label{fig:lens_multiple_sources}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{figs/H_vs_deltaT.png}
%    \caption{Simulated Roman survey distribution. Represents all of the pure astrometric events. The vertical line represents the approximate limiting magnitude of Roman (H~26). The two diagonal lines represent the 1 exposure (dashed line) and 100 exposure (solid line) curves.}
%    \label{fig:H_vs_deltaT}
%\end{figure}



% Significant Inputs
% 
% 
% 
% 

% Significant outputs
% tE
% theta_E
% 
% 

%The Nancy Grace Roman Space Telescope (Roman) has a revolutionary 0.1 mas of astrometric precision (for 100 exposures) \citet{Penny2019}. With this new level of astrometric precision, Roman will be able to resolve events no other telescope in history has been able to opening the door for true astrometric microlensing results

% (4a) Astro/Photo methods different (produce different observables)

%*******************


%Astrometric microlensing also produces different observables from photometric microlensing. Astrometric microlensing detects events at a larger t$_E$ than photometric causing one to detect many more events overall. The trade off is that you get less information from the event itself as astrometric microlensing doesn't constrain the $\pi_E$ parameter very well. 

% (4b) Astro/Photo different (Astrometric detects events with larger L/S Seperation)

%Astrometric microlensing's observables come in the form of $\theta_E$ and t$_E$. Astrometric L/S seperation is not as constrained as photometric L/S seperation. For Astrometric microlensing, events with nearby lenses, large u, are more common than events with small u meaning that a majority of astrometric events will have no photometric signal. 

% (4bI) Pruett2023 30Msol photometric simulation with u0< 2

%A paper was release recently by \citet{Pruett2022} where the simulation code PopSyCLE was used to estimate the PBH microlensing event detections with photometric parameters. Pruett primarily used pbhmass = 30Msun and events with a u0 > 2.

% (4bII) My simulations will be focused on everything not ^^

%This is a continuation of the work done by \citet{Pruett2022}, however for my simulations, I have specifically cut out all events with $u_0 < 2$ to cut out all photometrically detectable events. The goal is to compliment the work already done and specifically look at the astrometric readings of Roman. To do this, we have made specific cuts (mentioned more at [[SECTION]]) so that the data we get is distinct from \citet{Pruett2022}. We elaborate more on the cuts in Section 3.3. We also simulate many PBH masses between 10**-4 and 1000 to account for a variety of PBH mass theories and keep fDM = 1. 



%(Rough (Bullet Points?)) Dark Matter (DM) makes up $25\%$ of the energy density of the universe today, yet not much is known about it. Primordial Black Holes are one of the oldest models for dark matter. Primordial Black Holes (PBHs) are theoretical compact objects formed at the beginning of the universe due to density fluctuations. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Fig. \ref{fig:population} shows the projected sensitivity and projected constraints from this work with current PBH constraints in $f_{\rm DM}-m_{\rm PBH}$. In the most optimistic scenario where we assume that all PBH events can be exactly identified as such, we turn our PBH event rates described in Section \ref{sec:event_rates} into a $95\%$ confidence bound on detecting PBHs across $m_{\rm PBH}$, with the following,
%%
%\begin{equation}
%    \sigma_{f_{\rm DM}} \approx \frac{1}{N^{\rm PBH}}\,,
%\end{equation}
%where $N^{\rm PBH} $ is the expected number of PBH events from these simulations, separated by mass.
%This approximation equates to assuming the number of PBH microlensing events are described by Poisson statistics and assuming a model with $f_{\rm DM} = 1$.
%\perkins{Because of these very optimistic assumptions, this prediction is seen more as an estimate of the sensitivity than a prediction on the constraints attainable with RTS.}
%%
%In this maximally optimistic scenario, we find a peak sensitivity of the GBTDS to $f_{\rm DM}\approx3\times10^{-4}$ at $m_{\rm PBH}=1 M_{\odot}$. The sensitivity tapers to $f_{\rm DM}\approx10^{-1}$ and $f_{\rm DM}\approx10^{-2}$ at $m_{\rm PBH}=10^{-3}$ and $m_{\rm PBH}=10^{3}$, respectively. For $m_{\rm PBH}$ from $10^{-3}M_{\odot}-10^{3}M_{\odot}$ we predict that the GBTDS will sensitive at novel $f_{\rm DM}$ when compared with current photometric microlensing constraints \citep{Alcock2001,Tisserand2006,Wyrzykowski2011b, Blaineau2022}. Our sensitivity region in Fig. \ref{fig:population} suggests that the GBTDS may be able to fill the $m_{\rm PBH}=10^{-1}M_{\odot}-10^{3}M_{\odot}$ gap between microlensing and early universe cosmic microwave background constraints \citep{Ali-Haimoud2017,Ricotti2008} down to the $f_{\rm DM}\approx10^{-2}$ level. 
%
%\perkins{Note to authors: We are considering which of these predictions to include. This one might not be included. We are open to input.}
%Also shown in Fig. \ref{fig:population} is a more conservative sensitivity line from our analysis. This sensitivity line factors in PBH lens confusion with the astrophysical lenses by considering the same calculation as above, but focusing on the regions of high confidence, outlined in Sec.~\ref{sec:distinguishability} and statistics from that calculation shown graphically in Fig.~\ref{fig:mass_vs_prob}.
%Where the previous calculation was optimistic in that it assumed total discriminatory power between PBH and astronomical populations of lenses across the entire domain, this calculation is more realistic in that it focuses on the numbers of events expected in regions of parameter space where this assumption is much more likely to be valid (distinct regions of high probability to be a PBH lens).
%In this regime we have a peak sensitivity down to $f_{\rm DM}\approx X$ at $m_{\rm PBH}=X$, and are still sensitive to novel $f_{\rm DM}$ over previous photometric microlensing constraints in $m_{\rm PBH}=X M_{\odot}-XM_{\odot}$ ranges. 
%The actual PBH constraints derivable from the sample of astrometric microlensing events from the GBTDS are likely to be between the two sensitivity lines in Fig. \ref{fig:population}. 
%This is because confusion between PBHs and the astrophysical lens population can be modelled and accounted for using the methods of \cite{Perkins2023}.
%
%While the above two predictions are more related to the sensitivity of this probe to different mass ranges, we can also make a more careful, but still simplistic, prediction about the constraints themselves, by again using the Fisher information.
%Assuming the number of detected microlensing events is described by two independent Poisson processes, one described by the astrophysical model and one described by the PBH model, we can calculate the Fisher information on the parameter $f_{\rm DM}$ itself. 
%The expected number of PBH events from the second Poisson model will be parameterized as $f_{\rm DM} N^{\rm PBH}$, where $N^{\rm PBH} $ are the expected numbers of PBH events for the GBTD survey shown in Fig.~\ref{fig:event_rates}.
%This can then be translated to an estimate of the covariance of this number through the Cram\'er-Rao bound, leading to an estimated constraint on $f_{\rm DM}$ (at $95\%$ confidence) of (see App.~\ref{app:fisherNaive} for details on the derivation)
%\begin{equation}
%    f_{\rm DM}  \leq  1.96  \frac{\sqrt{N^{\rm Astro}}}{N^{\rm PBH}}\,,
%\end{equation}
%This prediction for the constraint includes the transformation from the $1\sigma$ estimate from the Fisher approximation to a $95\%$ confidence constraint, assuming a Gaussian posterior distribution on $f_{\text{DM}}$.
%It was also derived by assuming the null hypothesis, i.e., that $f_{\rm DM}=0$.
%Constraint predictions derived with this method are shown as the \textcolor{red}{COLOR} line. 
%Our prediction on the constraints range from $f_{\rm DM} \approx XX-YY$ in the mass range we examined, peaking at $f_{\rm DM} \approx XX$ for a PBH mass of $M_{\rm PBH} = YY$.
%
%\perkins{Note to authors: We are considering which of these predictions to include. This one might not be included. We are open to input.}
%As before, this approximation does not take into account that some events \emph{are more likely} to include PBH lenses rather than astrophysical ones. 
%By repeating this calculation, new constraint predictions can be derived specifically focused on the areas of parameter space that are distinctly dominated by PBH lenses (separated by mass).
%Similar to before, this calculation begins to fold in information about the parameters of the events, neglected in our first approximation.
%Constraint predictions derived with this method are shown as the \textcolor{red}{COLOR} line. 
%Our prediction on the constraints range from $f_{\rm DM} \approx XX-YY$ in the mass range we examined, peaking at $f_{\rm DM} \approx XX$ for a PBH mass of $M_{\rm PBH} = YY$.
%
%\perkins{Note to authors: Potential bonus analysis. This analysis is significantly more involved, but would be a lot more accurate and include full UQ for the estimate of $f_{\text{DM}}$. Also possible to jointly sample the astrophysical abundance and marginalize. This is exactly the restricted analysis from \citet{Perkins2023} and approximating the posteriors for the events with Fisher matrices, which is not the most accurate, but significantly improves on a fisher estimate on the constraint for $f_{\text{DM}}$. Open to input about how wanted this kind of result would be. }
%A final estimate of hierarchical effectiveness achievable with the data available takes into account the event parameter locations and uncertainty. 
%To do this, we must consider an inhomogeneous Poisson distribution for the population model, as opposed to the homogeneous one used in the past estimates, and we utilize the Fisher information estimates for the individual events computed earlier in this work. 
%With this new information, we can sample from the full posterior on $f_{\rm DM}$ directly, improving on the Fisher information estimate on $f_{\rm DM}$ used above.
%This is the ``restricted analysis'' of \citet{Perkins2023} while approximating the posterior distributions on the event parameters with Fishers, as opposed to fully sampling the event posteriors.
%While this analysis was shown to be sensitive to bias when using incorrect modeling assumptions in \citet{Perkins2023}, its use as a predictor with simulated data is useful as it roughly mimics the distributions from the fully robust analysis \citep[see Appendix~B of][]{Perkins2023} and is guaranteed to be bias-free as the underlying model is fully known with simulated data.
%The details of this calculation are shown in Appendix~\ref{app:fullfDMSampling}.
%Constraint predictions derived with this method are shown as the \textcolor{red}{COLOR} line. 
%Our prediction on the constraints range from $f_{\rm DM} \approx XX-YY$ in the mass range we examined, peaking at $f_{\rm DM} \approx XX$ for a PBH mass of $M_{\rm PBH} = YY$.



%\section{Population Constraint Predictions with Full Inhomogeneous Poisson}\label{app:fullfDMSampling}
%
%\emph{Stretch Goal}. Doing the full inhomogeneous Poisson likelihood might actually be feasible. We will have to neglect observation bias though, for sure.
%\begin{align}\nonumber
%    p(f_{\rm DM} | \{d_i\}, N^{\rm obs} , \Lambda)  &\propto e^{- N(f_{\rm DM} , \Lambda)} \left(N(f_{\rm DM} , \Lambda) \right)^{N^{\rm obs}} \prod_i^{N^{\rm obs}} \int p(d_i | \theta) p(\theta | f_{\rm DM} , \Lambda) d\theta \,,\\
%    &\propto e^{- \left( N^{\rm Astro} + f_{\rm DM } N^{\rm PBH} \right)} \left(N^{\rm Astro} + f_{\rm DM } N^{\rm PBH} \right)^{N^{\rm obs}} \\
%    &\times \prod_i^{N^{\rm obs}} \int \mathcal{N}(\theta| \mu=\theta^{\rm inj}, \Sigma = \Gamma^{-1}) \left( p(\theta|{\rm PBH}) f_{\rm DM} \psi_{\rm DM} + p(\theta | {\rm Astro}) ( 1- f_{\rm DM} \psi_{\rm DM}) \right) d\theta\\
%    &\propto e^{- \left( N^{\rm Astro} + f_{\rm DM } N^{\rm PBH} \right)}\left(N^{\rm Astro} + f_{\rm DM } N^{\rm PBH} \right)^{N^{\rm obs}} \\
%    &\times \prod_i^{N^{\rm obs}} \left( \hat{P}_{\rm PBH} f_{\rm DM} \psi_{\rm DM} + \hat{P}_{\rm Astro} ( 1- f_{\rm DM} \psi_{\rm DM}) \right) 
%\end{align}
%where the $\hat{P}$ variables are the respective integrals and $\psi_{\rm PBH}$ is the relative abundance of PBHs at $f_{\rm DM} = 1$.
%Things that make this pretty straightforward to do, actually, is that \texttt{SciPy}'s KDE already has an "integrate gaussian" function, which can exactly (analytically) do the integral above, $\hat{P}$. This would require full, numerical sampling, though. Similar to the "restricted" analysis from the last paper though, we can precompute all the intergrals and \emph{very} quickly perform the sampling, because it's just doing weighted sums at that point.
%
%\begin{align}
%    \ln p(f_{\rm DM} | \{d_i\}, N^{\rm obs} , \Lambda) &\propto -\left( N^{\rm Astro} + f_{\rm DM } N^{\rm PBH} \right) +N^{\rm obs} \ln \left(N^{\rm Astro} + f_{\rm DM } N^{\rm PBH} \right) \\
%    &+\sum_i^{N^{\rm obs}} \ln \left(\hat{P}_{\rm PBH} f_{\rm DM} \psi_{\rm DM} + \hat{P}_{\rm Astro} ( 1- f_{\rm DM} \psi_{\rm DM}) \right) \,,
%\end{align}
